Topological phases in two-legged Heisenberg ladders with alternating interactions

We analyze the possible existence of topological phases in two-legged spin ladders considering a staggered interaction in both chains. When the staggered interaction in one chain is shifted by one site with respect to the other chain, the model can be mapped, in the continuum limit, into a non linear sigma model NL$\sigma$M plus a topological term which is nonvanishing when the number of legs is two. This implies the existence of a critical point which distinguishes two phases. We perform a numerical analysis of energy levels, parity and string non-local order parameters, correlation functions between $x,y,z$ components of spins at the edges of an open ladder, the degeneracy of the entanglement spectrum and the entanglement entropy in order to characterize these two different phases. Finally, we identify one phase with a Mott insulator and the other one with a Haldane insulator.

==> bibliografia.tex <==
\begin{thebibliography}{10}

% INTRODUZIONE

\bibitem{Hohenberg}  
P. C. Hohenberg, \textit{Phys.Rev.} \textbf{158}:383, 1967.

\bibitem{MerminWagner}
N.D.Mermin and H.Wagner, \textit{Phys.Rev.Lett.} \textbf{17}:1133, 1966.

\bibitem{Berezinskii}
V. L. Berezinskii, \textit{Sov.Phys.JEPT} \textbf{34}:610, 1972.

\bibitem{KosterliztThoulesse}
J. M. Kosterlitz and D. J. Thoulesse, \textit{J.Phys.C} \textbf{6}:1181, 1973. 

\bibitem{Affleck1}
I. Affleck, \textit{Phys.Rev.Lett.} \textbf{54}:966, 1985.

\bibitem{Haldane1}
F. D. M. Haldane, \textit{Phys.Lett.A} \textbf{93}:464, 1983.

\bibitem{Haldane2}
F. D. M. Haldane, \textit{Phys.Rev.Lett.} \textbf{50}:1153, 1983.

\bibitem{Affleck2}
I. Affleck, \textit{Fields, strings and critical phenomena} (E. Berezin and J. Zinn-Justin ed.s North-Holland, 1990).

\bibitem{Rajaraman}
R. Rajaraman, \textit{Solitons and instantons} (North-Holland, 1982).

\bibitem{Morandi}
G. Morandi, \textit{The role of topology in classical and quantum physics} (Springer-Verlac, 1992).

\bibitem{Polyakof}
A. M. Polyakof, \textit{Phys.Lett. B} \textit{59}:79, 1975.

\bibitem{ShankarRead}
R. Shankar and N.Read, \textit{Nucl.Phys.B} \textbf{336}:457, 1990.

\bibitem{AffleckKennedyLiebTasaki1}
I. Affleck, T. Kennedy, E. H. Lieb and H. Tasaki, \textit{Phys.Rev.Lett.} \textbf{59}:799, 1987.

\bibitem{AffleckKennedyLiebTasaki2}
I. Affleck, T. Kennedy, E. H. Lieb and H. Tasaki, \textit{Cmmun.Math.Phys.} \textbf{115}:477, 1988.

\bibitem{KennedyTasaki}
T. Kennedy and H. Tasaki, \textit{Phys.Rev.B} \textbf{45}:304, 1992.

\bibitem{PollmannTurnerBergOshikawa}
F. Pollmann, A. M. Turner, E. Berg and M. Oshikawa, \textit{Phys.Rev.B} \textbf{81}:064439, 2010.

\bibitem{GuWen}
Z.-C. Gu and X.-G. Wen, \textit{Phys.Rev.B} \textbf{80}:155131, 1990.

\bibitem{Haldane3}
F. D. M. Haldane, \textit{Phys.Rev.Lett.} \textbf{61}:1029, 1988.

\bibitem{FradkinStone}
E. Fradkin and M. Stone, \textit{Phys.Rev.B} \textbf{38}:7215, 1988.

\bibitem{IoffeLarkin}
L. B. Ioffe and A. I. Larkin, \textit{Int.J.Mod.Phys.B} \textbf{2}:203, 1988.

\bibitem{DombreRead}
T. Dombre and N. Read, \textit{Phys.Rev.B} \textbf{38}:7181, 1988.

\bibitem{AngelucciJug}
A. Angelucci and G. Jug, \textit{Int.J.Mod.Phys.B} \textbf{3}:1069, 1989.

\bibitem{RiceGolapanSigrist} 
T. M. Rice, S. Golapn and M. Sigrist, \textit{Europhys. Letters} \textbf{23}:445, 1993.

\bibitem{DagottoRieraScalapino}
E. Dagotto, J. Riera and D. Scalapino, \textit{Phys.Rev.B} \textbf{45}:5744, 1992.

\bibitem{Dagotto}
E. Dagotto, \textit{Rev.Mod.Phys.} \textbf{66}:763, 1994.

\bibitem{JohnstonJohnstonGoshornJacobsen}
D. C. Johnston, J. W. Johnston, D. P. Goshorn and A. J. Jacobsen, \textit{Phys.Rev.B} \textbf{35}:219, 1987.

\bibitem{HiroiAzumaTakanoBando}
Z. Hiroi, M. Azuma, M. Takano, and Y. Bando, \textit{J.Solid State Chem.} \textbf{95}:230, 1991.

\bibitem{Azuma}
M. Azuma et al, \textit{Phys.Rev.Lett.} \textbf{73}:3463, 1994.

\bibitem{BarnesRiera}
T. Barnes and J. Riera, \textit{Phys.Rev.B} \textbf{50}:6817, 1994.

\bibitem{DagottoRice}
E. Dagotto and T. M. Rice, \textit{Science} \textbf{271}:618, 1996.

\bibitem{Khveshchenko}
D. V. Khveshchenko, \textit{Phys.Rev.B} \textbf{52}:15319, 1995.

\bibitem{Senechal} 
D. S$\acute{e}$n$\acute{e}$chal, \textit{Phys.Rev.B} \textbf{52}:15319, 1995.

\bibitem{ArringaErcolessiMorandiPieriRoncaglia}
S.Dell'Aringa, E.Ercolessi, G.Morandi, P.Pieri, and M.Roncaglia, \textit{Phys.Rev.Lett.} \textbf{78}:2457, 1997.

\bibitem{Sierra1} 
G. Sierra, \textit{J.Phys. A: Math. Gen.} \textbf{29}:3299, 1996.

\bibitem{Sierra2} 
G. Sierra, \textit{con-mat/9610057}.

\bibitem{KlauderSkagerstam} 
J. R. Klauder and B. S. Skagerstam, \textit{Coherent states} (World Scientific, 1984).

\bibitem{MontorsiRoncaglia}
A. Montorsi and M. Roncaglia, \textit{Phys.Rev.Lett.} \textbf{109}:236404, 2012.

\bibitem{BarbieroMontorsiRoncaglia}
L. Barbiero, A. Montorsi and M. Roncaglia, \textit{Phys.Rev.B} \textbf{88}:035109, 2013.

\bibitem{SchnyderRyuFurusakiLudwig}
A. P. Schnyder, S. Ryu, A. Furusaki and A. W. W. Ludwig,\textit{Phys.Rev.B} \textbf{78}:195125, 2008.

\bibitem{Kitaev}
A. Kitaev, \textit{Conf.Proc.} \textbf{1134}:22, 2009.

\bibitem{Wen}
X.-G. Wen, \textit{Phys.Rev.B} \textbf{85}:085103, 2012.

\bibitem{FidkowskiKitaev} 
L.Fidkowski and A.Kitaev,\textit{Phys.Rev.B} \textbf{81}:134509, 2010.

\bibitem{MontorsiDolciniIottiRossi}
A. Montorsi, F.Dolcini, R.Iotti and F.Rossi, \textit{Phys.Rev.B} \textbf{95}:245108, 2017

\bibitem{MartinShankarSierra}
M.A. Martin-Delgrado, R. Shankar and S.Sierra, \textit{Phys.Rev.Lett.} \textbf{77}:3443, 1996.

% PARTE ANALITICA

\bibitem{Auerbach}
A. Auerbach, \textit{Interacting Electrons and Quantum Magnetism} {Springer, 2 edition, 1998}.

\bibitem{Fradkin} 
E. Fradkin, \textit{Field Theories of Condensed Matter Systems} {Addison-Wesley, 1 edition, 1991}.

\bibitem{GreveBirgeneauWiese} 
M. Greven, R, J. Birgeneau and U.-J. Wiese, \textit{Phys.Rev.Lett.} \textbf{77}:1865, 1996.

\bibitem{WhiteNoackScalapino} 
S. R. White, R. M. Noack and D. J. Scarpino, \textit{Phys.Rev.Lett.} \textbf{73}:886, 1994.

\bibitem{DMRG2}
S.R. White, \textit{Phys.Rev.B} \textbf{48}:10345, 1993.

\bibitem{DMRG1}
S.R. White, \textit{Phys.Rev.} \textbf{69}:2863, 1992.

\bibitem{ver}
F. Verstraete, J.I. Cirac, V. Murg, \textit{Adv.Phys.} \textbf{57}:143, 2008.

\bibitem{sch}
U. Schollw$\ddot{o}$ck \textit{Ann.Phys.} \textbf{326}:96, 2011.

\bibitem{TN}
R.Or$\acute{u}$s \textit{Ann.Phys.} \textbf{349}:117-158, 2014.




\end{thebibliography}
